Large language models for aspect-based sentiment analysis

Large language models (LLMs) offer unprecedented text completion capabilities. As general models, they can fulfill a wide range of roles, including those of more specialized models. We assess the performance of GPT-4 and GPT-3.5 in zero shot, few shot and fine-tuned settings on the aspect-based sentiment analysis (ABSA) task. Fine-tuned GPT-3.5 achieves a state-of-the-art F1 score of 83.8 on the joint aspect term extraction and polarity classification task of the SemEval-2014 Task 4, improving upon InstructABSA [@scaria_instructabsa_2023] by 5.7%. However, this comes at the price of 1000 times more model parameters and thus increased inference cost. We discuss the the cost-performance trade-offs of different models, and analyze the typical errors that they make. Our results also indicate that detailed prompts improve performance in zero-shot and few-shot settings but are not necessary for fine-tuned models. This evidence is relevant for practioners that are faced with the choice of prompt engineering versus fine-tuning when using LLMs for ABSA.

==> _extensions/mikemahoney218/arxiv/partials/_authors.tex <==
$-- You can use as many custom partials as you need. Convention is to prefix name with '_'
$-- It can be useful to use such template to split some template parts in smaller pieces, which is easier to reuse.
$-- This '_custom.tex' is used on 'title.tex' as example.
$-- See other existing format in quarto-journals/ organisation.
$-- %%%% TODO %%%%%
$-- Use it if you need to insert content at this specific place of the main Pandoc's template. Otherwise, remove it.
$-- Here we are using it to format the authors part of the template.
$-- %%%%%%%%%%%%%%%

\textbf{$it.name.literal$}$if(it.orcid)$~\orcidlink{$it.orcid$}$endif$$for(it.affiliations/first)$\\$it.department$\\$it.name$\\$if(it.city)$$it.city$$if(it.postal-code)$,\ $it.postal-code$$endif$$endif$$endfor$\\$if(it.email)$\href{mailto:$it.email$}{$it.email$}$endif$


==> _extensions/mikemahoney218/arxiv/partials/before-body.tex <==
$-- Implements the frontmatter, title page, and abstract.
$--
$-- %%%% TODO %%%%%
$-- Customize is needed, otherwise remove this partials to use Quarto default one
$-- %%%%%%%%%%%%%%%%
$if(has-frontmatter)$
\frontmatter
$endif$
$if(title)$
$if(beamer)$
\frame{\titlepage}
$else$
\maketitle
$endif$
$if(abstract)$
\begin{abstract}
$abstract$
\end{abstract}
$endif$
$endif$
$if(keywords)$
{\bfseries \emph Keywords}
\def\sep{\textbullet\ }
$for(keywords/allbutlast)$$keywords$ \sep $endfor$
$for(keywords/last)$$keywords$$endfor$

$endif$


==> _extensions/mikemahoney218/arxiv/partials/title.tex <==
$-- Provides configuration of document metadata for writing the title block.
$-- Note that in addition to these templates and partials, Quarto will also make normalized authors and affiliations data available to the template,
$-- making is easy to write custom title blocks against a standard schema.
$--
$-- %%%% TODO %%%%%
$-- Customize is needed, like below for printing the authors. Otherwise remove this partials to use Quarto default one.
$-- %%%%%%%%%%%%%%%%
$if(linenumbers)$
\usepackage{lineno}
\linenumbers
$endif$
$if(doublespacing)$
\usepackage{setspace}
\doublespacing
$endif$
$if(date)$
\renewcommand{\today}{$date$}
$endif$
\newcommand{\runninghead}{A Preprint }
$if(runninghead)$
\renewcommand{\runninghead}{$runninghead$ }
$endif$
$if(title)$
\title{$title$$if(thanks)$\thanks{$thanks$}$endif$}
$endif$
$if(subtitle)$
\usepackage{etoolbox}
\makeatletter
\providecommand{\subtitle}[1]{% add subtitle to \maketitle
  \apptocmd{\@title}{\par {\large #1 \par}}{}{}
}
\makeatother
\subtitle{$subtitle$}
$endif$
\author{${ by-author:_authors.tex()[\\\\\\] }}
\date{$date$}

